Predicting the Road Ahead: A Knowledge Graph based Foundation Model for Scene Understanding in Autonomous Driving

The autonomous driving field has seen remarkable advancements in various topics, such as object recognition, trajectory prediction, and motion planning. However, current approaches face limitations in effectively comprehending the complex evolutions of driving scenes over time. This paper proposes FM4SU, a novel methodology for training a symbolic foundation model (FM) for scene understanding in autonomous driving. It leverages knowledge graphs (KGs) to capture sensory observation along with domain knowledge such as road topology, traffic rules, or complex interactions between traffic participants. A bird's eye view (BEV) symbolic representation is extracted from the KG for each driving scene, including the spatio-temporal information among the objects across the scenes. The BEV representation is serialized into a sequence of tokens and given to pre-trained language models (PLMs) for learning an inherent understanding of the co-occurrence among driving scene elements and generating predictions on the next scenes. We conducted a number of experiments using the nuScenes dataset and KG in various scenarios. The results demonstrate that fine-tuned models achieve significantly higher accuracy in all tasks. The fine-tuned T5 model achieved a next scene prediction accuracy of 86.7%. This paper concludes that FM4SU offers a promising foundation for developing more comprehensive models for scene understanding in autonomous driving.

==> sections/05_implementation.tex <==
\section{Implementation}

The Text-to-Text Transfer Transformer (T5) model, as outlined in the paper ``Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer'' \cite{1910.10683}, represents a significant leap in natural language processing technology. This model is built on the principle of converting all NLP tasks into a unified text-to-text format, simplifying the training process and enhancing the model's adaptability to various tasks. This is a good fit to our project ideology of converting autonomous driving scene into text format and make prediction in text format as well.

\subsection{Application of T5 in Scene Understanding}
In the context of autonomous driving scene understanding, the T5 model's capacity for multi-token predictions is particularly advantageous and is why it is chosen over the other masked language models such as RoBERTa. Unlike other models that predict a single token per mask token, T5 can generate multiple tokens for a single mask token (thus, multiple entities predicted for a single masked area) in the scene representation. This feature aligns perfectly with the nature of driving scenes, where each area might contain several entities (e.g., vehicles, pedestrians, road signs) or none at all (represented by <empty> token). This multi-token prediction capability of T5 is crucial for capturing the dynamic nature of driving environments.


\subsection{Implementation Details}
For this project, T5's inherent flexibility and its pre-training on large scale of data such as the ``Colossal Clean Crawled Corpus'' (C4) \cite{2104.08758} are leveraged to fine-tune the model on a specialized task. The model is adapted to interpret a matrix-based representation of driving scenes, where each cell in the matrix corresponds to a specific area around the ego vehicle in the real world. The challenge lies in predicting the contents of these areas, when masked, to understand and anticipate the driving context accurately.

The input format for the T5 model in this scenario is a serialized string of tokens representing different aspects of a driving scene, including spatial layout, existing entities, and environmental conditions. Mask tokens are introduced in place of the areas to be predicted. The T5 model is then tasked with predicting the entities within these masked areas. For detailed illustration, see \ref{fig:T5_ex}.


\begin{figure}[h]
\centering
\begin{tikzpicture}
  % Node for the T5 sample image on the left
  \node (t5_sample) {\includegraphics[width=0.3\textwidth]{images/t5_sample.png}};
  
  % Node for the custom formatted text on the right with smaller font size
  \node[right=0cm of t5_sample] (custom_format) {
    \begin{minipage}{0.6\textwidth}
      \scriptsize % This will make the text smaller
      \textbf{Original matrix representation sequence} \\
      <country> US <dist> 4.8 <orientation\_diff> 0 <scene\_start> lane <col\_sep> lane <concept\_sep> car <col\_sep> \textcolor{red}{pedestrian crossing} <col\_sep> walkway <row\_sep> ... <col\_sep> \textcolor{red}{intersection} <col\_sep> <turn stop area> <col\_sep> ... \\
      \\
      \textbf{Input masked matrix representation sequence} \\
      <country> US <dist> 4.8 <orientation\_diff> 0 <scene\_start> lane <col\_sep> lane <concept\_sep> car <col\_sep> \textcolor{red}{<X>} <col\_sep> walkway <row\_sep> ... <col\_sep> \textcolor{red}{<Y>} <col\_sep> <turn stop area> <col\_sep> ... \\
      \\
      \textbf{Targets} \\
      \textcolor{red}{<X>} \textcolor{red}{pedestrian crossing} \textcolor{red}{<Y>} \textcolor{red}{intersection} \textcolor{red}{<Z>}
    \end{minipage}
  };
\end{tikzpicture}
\caption{Illustration of input, output of the specific masked language modeling}
\tiny\raggedright On the left is the original example from T5 paper. On the right is the specific task of this project. Note that <X> <Y> <Z> were used for easier interpretation. T5 actually supports mask tokens in the form of <extra\_id\_n> tokens, where n can go from 0 to 99 (thus up to 100 masked tokens). Note that for extreme cases where more than 100 areas needed to be masked, we only mask the less than $100$ central areas around ego vehicle. <country> <dist> <orientation\_diff> tokens indicate respectively the nature of the following tokens being country, distance traveled and orientation difference between ego vehicle in pair of scenes. <col\_sep> <row\_sep> are position delimiter delimiting columns and rows of the matrix, implicitly preserving the geo-spatial structure of the scene. <concept\_sep> delimits different map concepts/entities within an area. This kind of tokenization is result of optimized tokenization (details in Chapter 6).
\label{fig:T5_ex}
\end{figure}
